Rethinking Offensive Text Detection as a Multi-Hop Reasoning Problem

We introduce the task of implicit offensive text detection in dialogues, where a statement may have either an offensive or non-offensive interpretation, depending on the listener and context. We argue that reasoning is crucial for understanding this broader class of offensive utterances and release SLIGHT, a dataset to support research on this task. Experiments using the data show that state-of-the-art methods of offense detection perform poorly when asked to detect implicitly offensive statements, achieving only ${\sim} 11\%$ accuracy. In contrast to existing offensive text detection datasets, SLIGHT features human-annotated chains of reasoning which describe the mental process by which an offensive interpretation can be reached from each ambiguous statement. We explore the potential for a multi-hop reasoning approach by utilizing existing entailment models to score the probability of these chains and show that even naive reasoning models can yield improved performance in most situations. Furthermore, analysis of the chains provides insight into the human interpretation process and emphasizes the importance of incorporating additional commonsense knowledge.

==> tables/fact_verification.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{F-1 Score} \\
    \cline{2-4}
    & SUP & REF & NEI \\
    \midrule
    KernalGAT &  0.46 & 0.22 & 0.38\\
    CorefBERT &  0.42 & 0.23 & 0.38\\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:fact_results}
\end{table}

==> tables/tab_ex_2_1.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{rcc}
%     \toprule
%     & \multicolumn{2}{c}{\textbf{Entailment Scores}} \\
%     \cline{2-3}
%     \textbf{Steps} & RoBERTa & DeBERTa\\
%     \midrule
%          $s_0 \rightarrow s_1$ &  \textbf{0.861} & \textbf{0.831}\\
%          $s_0 \rightarrow s_l$ & 0.067 & 0.039 \\
%     \bottomrule
%     \end{tabular}
%     \caption{The entailment scores from first step to second step versus first step to last step in the chain. The higher the scores are, the better the previous steps can entail the next steps. $s_0 \rightarrow s_1$: implicit insult to first step. $s_1 \rightarrow s_l$: implicit insult to last step.}
%     \label{tab:first_last}
% \end{table}

\begin{table}[t]
    \begin{subtable}{.48 \textwidth}
        
    
        \centering
        \begin{tabular}{rcc}
        \toprule
        & \multicolumn{2}{c}{\textbf{Entailment Scores}} \\
        \cline{2-3}
        \textbf{Steps} & RoBERTa & DeBERTa\\
        \cline{1-3}
             $s_0 \rightarrow s_1$ &  \textbf{86.1} & \textbf{83.1}\\
             $s_0 \rightarrow s_L$ & \phantom{0}6.7 & \phantom{0}3.9 \\
        \bottomrule
        \end{tabular}
        \caption{ }
        % \caption{The entailment scores from first step to second step versus first step to last step in the chain. The higher the scores are, the better the previous steps can entail the next steps. } %$s_0 \rightarrow s_1$: implicit insult to first step. $s_1 \rightarrow s_l$: implicit insult to last step.}
        \label{tab:first_last}
    
    \end{subtable}
    
    \begin{subtable}{.48\textwidth}
        \centering
        \begin{tabular}{rcc}
        \toprule
        & \multicolumn{2}{c}{\textbf{Contradiction Scores}} \\
        \cline{2-3}
        \textbf{Steps} & RoBERTa & DeBERTa\\
        \cline{1-3}
             $implicit \rightarrow non$ & 13.7          & 17.9\\
             $explicit \rightarrow non$ & \textbf{94.6} & \textbf{97.0} \\
        \bottomrule
        \end{tabular}
        \caption{ }
        % \caption{The contradiction scores from implicit statement to non-offensive statement versus explicit statement to non-offensive statement. Explicit statements are easier to be classified as ``contradiction'' to non-offensive statements.} %$s_0 \rightarrow s_1$: implicit insult to first step. $s_1 \rightarrow s_l$: implicit insult to last step.}
        \label{tab:contradiction}
    \end{subtable}
    \label{tab:entail_contrad}
    \caption{The entailment scores (a) and contradiction scores (b) from implicit statements to non-offerensive statements versus explicit statements to non-offensive statements.}
\end{table}

==> tables/tab_ex_2_2.tex <==

\begin{table*}[]
    \centering
    \begin{tabular}{rcccccccccc}
    \toprule
    & \multicolumn{10}{c}{\textbf{Entailment Scores}} \\
    \cmidrule(lr){2-11}
    & \multicolumn{5}{c}{\textbf{\small RoBERTa}}            & \multicolumn{5}{c}{\textbf{\small DeBERTa}}\\
    \cmidrule(lr){2-6}\cmidrule(lr){7-11}
    & \multicolumn{4}{c}{\small Chain Length} & {\small ALL} & \multicolumn{4}{c}{\small Chain Length} & {\small ALL} \\
    \cmidrule(lr){2-5} \cmidrule(lr){7-10}
    \textbf{Reasoning Model} & \small 3 &  \small 4 & \small 5 & \small 6 & & \small 3 & \small 4 & \small 5 & \small 6 & \\
    \midrule
    
    \textit{MUL} & 14.3  & \textbf{13.1} & \textbf{\phantom{0}4.6} & \phantom{0}5.4  & \textbf{11.5} & \textbf{12.1} & \textbf{\phantom{0}7.7}  & \phantom{0}1.8 & \phantom{0}3.3 & \textbf{\phantom{0}6.8}\\
    \textit{$E_{s_0 \rightarrow s_l}$} & \textbf{17.2}  & \phantom{0}9.1 & \phantom{0}4.4 & \textbf{\phantom{0}5.6} & \phantom{0}7.6 & \phantom{0}8.3 & \phantom{0}5.9 & \textbf{\phantom{0}2.4} & \textbf{\phantom{0}3.6} & \phantom{0}4.5\\ 
    \cmidrule(lr){1-11}
    
    \textit{MUL (k+)} & \textbf{38.1} & \textbf{32.0} & \textbf{17.9} & \textbf{16.5} & \textbf{23.5} & \textbf{30.2} & \textbf{20.3}  & \textbf{\phantom{0}7.6}  & \phantom{0}4.0 & \textbf{14.1} \\
    \textit{$E_{s_0 \rightarrow s_l}$ (k+)} & 35.9 & 15.9 & 10.8 & \phantom{0}8.6 & 15.0 & 25.3 & 11.9   & \phantom{0}7.5  & \textbf{\phantom{0}6.6} & 10.9\\ 
    
    \bottomrule
    \end{tabular}
    \caption{Entailment scores from the reasoning models, $MUL$ and $s_0 \rightarrow s_l$, as well as the accuracy calculated with the OTD models.  Column headers indicate subsets of the data, where all chains are of 3, 4, 5, or 6 steps respectively. \textit{k+}: scores indicate those where external knowledge is concatenated to all statements prior to a KIR step.}
    \label{tab:step_step_scores}
\end{table*}

==> tables/tab_example.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c}
    \toprule
    \textbf{Attribute} 
    \midrule
         I love bookclubs, I go every week. \\
    \midrule
    
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/tab_rule_stat.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc}
    \toprule
    \textbf{Rule} & \textbf{Times Applied} \\
    \midrule
         ASR   & 240 \\
         KIR   & 273 \\
         RR    & 756 \\ \hline
         Total & 1,269 \\
    \bottomrule
    \end{tabular}
    \caption{Different rules and the times they are applied to create chain of reasoning in the subset.}
    \label{tab:rules}
\end{table}
